Templates for 3D Object Pose Estimation Revisited: Generalization to New Objects and Robustness to Occlusions

We present a method that can recognize new objects and estimate their 3D pose in RGB images even under partial occlusions. Our method requires neither a training phase on these objects nor real images depicting them, only their CAD models. It relies on a small set of training objects to learn local object representations, which allow us to locally match the input image to a set of "templates", rendered images of the CAD models for the new objects. In contrast with the state-of-the-art methods, the new objects on which our method is applied can be very different from the training objects. As a result, we are the first to show generalization without retraining on the LINEMOD and Occlusion-LINEMOD datasets. Our analysis of the failure modes of previous template-based approaches further confirms the benefits of local features for template matching. We outperform the state-of-the-art template matching methods on the LINEMOD, Occlusion-LINEMOD and T-LESS datasets. Our source code and data are publicly available at https://github.com/nv-nguyen/template-pose

==> sections/4a_qualitative.tex <==
\begin{figure*}
% \newlength{\imageheight}

\setlength\imageheight{1.4cm}
\centering
\setlength\lineskip{1.pt}
\setlength\tabcolsep{1.pt} 
{\small
\begin{tabular}{c}
\begin{tabular}{
>{\centering\arraybackslash}m{1.cm}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{0.2cm}
>{\centering\arraybackslash}m{1.cm}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{\imageheight}
}
 & 
\includegraphics[height=\imageheight, ]{images/qualitative/unseen_duck_query.png}&
\includegraphics[height=\imageheight, ]{images/qualitative/unseen_duck_gt.png}&
\includegraphics[height=\imageheight, ]{images/qualitative/unseen_duck_balnas.png}&
\includegraphics[height=\imageheight, ]{images/qualitative/unseen_duck_ours.png} &
\includegraphics[height=\imageheight,
]{images/qualitative/unseen_duck_with_o.png}&
&
 &
\includegraphics[height=\imageheight, ]{images/qualitative/occ_driller_query.png} &
\includegraphics[height=\imageheight, ]{images/qualitative/occ_driller_gt.png}&
\includegraphics[height=\imageheight, ]{images/qualitative/occ_driller_wohlhart.png}&
\includegraphics[height=\imageheight, ]{images/qualitative/occ_driller_ours.png}&
\includegraphics[height=\imageheight]{images/qualitative/occ_driller_sim_occ.png}\\

\end{tabular}\\

\begin{tabular}{
>{\centering\arraybackslash}m{1.cm}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{0.2cm}
>{\centering\arraybackslash}m{1.cm}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{\imageheight}
}
\raisebox{0.0\height}{\rotatebox[origin=c]{90}{\bf \parbox{1.2cm}{Unseen}}} & 
\includegraphics[height=\imageheight, ]{images/qualitative/unseen_cat_query.png} &
\includegraphics[height=\imageheight, ]{images/qualitative/unseen_cat_gt.png}&
\includegraphics[height=\imageheight, ]{images/qualitative/unseen_cat_wohlhart.png}&
\includegraphics[height=\imageheight, ]{images/qualitative/unseen_cat_ours.png}&
\includegraphics[height=\imageheight]{images/qualitative/unseen_cat_sim.png}&
&
\raisebox{0.99\height}{\rotatebox[origin=c]{90}{\bf \parbox{1.2cm}{Unseen occluded}}} 

 &
\includegraphics[height=\imageheight, ]{images/qualitative/occ_cat_query.png} &
\includegraphics[height=\imageheight, ]{images/qualitative/occ_cat_gt.png}&
\includegraphics[height=\imageheight, ]{images/qualitative/occ_cat_balnas.png}&
\includegraphics[height=\imageheight, ]{images/qualitative/occ_cat_ours.png}&
\includegraphics[height=\imageheight]{images/qualitative/occ_cat_ours_with_o.png}\\
\end{tabular}\\

\begin{tabular}{
>{\centering\arraybackslash}m{1.cm}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{0.2cm}
>{\centering\arraybackslash}m{1.cm}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{\imageheight}
>{\centering\arraybackslash}m{\imageheight}
}
 & 
\includegraphics[height=\imageheight, ]{images/qualitative/unseen_eggbox_query.png} &
\includegraphics[height=\imageheight, ]{images/qualitative/unseen_eggbox_gt.png}&
\includegraphics[height=\imageheight, ]{images/qualitative/unseen_eggbox_balnas.png}&
\includegraphics[height=\imageheight, ]{images/qualitative/unseen_eggbox_ours.png}&
\includegraphics[height=\imageheight]{images/qualitative/unseen_eggbox_sim_occ.png}&
&
&
\includegraphics[height=\imageheight, ]{images/qualitative/occ_eggbox_query.png} &
\includegraphics[height=\imageheight, ]{images/qualitative/occ_eggbox_gt.png}&
\includegraphics[height=\imageheight, ]{images/qualitative/occ_eggbox_balnas.png}&
\includegraphics[height=\imageheight, ]{images/qualitative/occ_egg_box_ours.png}&
\includegraphics[height=\imageheight]{images/qualitative/occ_eggbox_ours_with_o.png}\\
& Query & GT & \cite{balntas-iccv17-poseguidedrgbdfeaturelearning} & Ours & Similarity  &  & & Query & GT & \cite{balntas-iccv17-poseguidedrgbdfeaturelearning} & Ours & Similarity
\end{tabular}
\end{tabular}
}
\vspace{-3mm}
\caption{{\bf Qualitative results on \emph{unseen} objects} of LINEMO (left) and Occlusion LINEMOD (right) on Split~\#2. Our method retrieves the correct template and pose while \cite{balntas-iccv17-poseguidedrgbdfeaturelearning} fails on \emph{unseen} objects, particularly in the presence of occlusion.
%As can be shown, while previous works~\cite{balntas-iccv17-poseguidedrgbdfeaturelearning} fails to generalize on \emph{unseen objects}, particularly in the presence of occlusion, our method is still able to retrieve correct template.
}
\end{figure*}

==> tables/ablation_hash_tables.tex <==
\begin{table}[!t]
\addtolength{\tabcolsep}{-1pt}
% \rowcolors{2}{white}{gray!10}
%\rowcolors{5}{gray!10}{}
\centering
    \scalebox{0.85}{
    \begin{tabular}{l c c c c c c c}
	\toprule
	\multirow{2}{*}{\bf DBSCAN} & \multicolumn{2}{c}{\textbf{AccHash}}  & \multicolumn{2}{c}{\textbf{Acc15}}  & \multicolumn{2}{c}{\textbf{Tradeoff(\%)}} \\
	&  Seen & Unseen  & Seen & Unseen & Seen & Unseen \\
	\midrule
	$\epsilon$=0.05, min=2 & 92.2 & 99.7 & - & - & 10.2 & 41.7\\
	$\epsilon$=0.05, min=5 & 77.5 & 91.0 & - & - & 4.7 & 25.9\\
% 	$\epsilon$=0.10, min=1 & 77.5 & - & - & - & 4.7 & -\\
% 	$\epsilon$=0.10, min=2 & 77.5 & - & - & - & 4.7 & -\\
% 	$\epsilon$=0.10, min=5 & 77.5 & - & - & - & 4.7 & -\\
	
	
    \bottomrule
    \end{tabular}} 
\vspace*{-1mm}
\caption{Ablation study on hashing tables}

\label{tab:linemod_full_err}
\end{table}


==> tables/tless.tex <==
\begin{table}[t]
	\centering
    \resizebox{0.95\linewidth}{!}{
	\begin{tabular}{@{}l c c c c@{}}
	\toprule
    % \multirow{2}{*}{\bf Method} & \multirow{2}{*}{\bf Bounding boxes} & \multicolumn{3}{c}{\textbf{Recall VSD}}\\
    \multirow{2}{*}{\bf Method} & \multirow{2}{*}{\bf \parbox{1.3cm}{Bounding boxes}} & \multicolumn{3}{c}{\textbf{Recall VSD}}\\
	\cmidrule(lr){3-5}                                
	& & \textbf{Obj. 1-18} & \textbf{Obj. 19-30} & \textbf{Average} \\
	\midrule
	Implicit \cite{sundermeyer-eccv18-implicit3dorientationlearning} & GT & 35.60 & 42.45 & 38.34\\
	MultiPath \cite{sundermeyer-cvpr20-multipathlearning} & GT  & 35.25 & 33.17 & 34.42\\
	Ours & GT & \bf 58.62 & \bf 58.44 & \bf 58.54\\
	\midrule
	Ours & Pix2Pose~\cite{park-iccv19-pix2pose} & 40.16 & 33.70 & 37.54\\
	\bottomrule
	\end{tabular}}
	\vspace{-3mm}	\caption{{Comparison with \cite{sundermeyer-eccv18-implicit3dorientationlearning, sundermeyer-cvpr20-multipathlearning} on trained objects (objects 1-18)} and ``untrained'' objects (objects 19-31) of T-LESS using the protocol from [30]. We use the same ResNet50 backbone and learning rate schedules as for LINEMOD. \cite{sundermeyer-eccv18-implicit3dorientationlearning, sundermeyer-cvpr20-multipathlearning} only report results using the GT bounding boxes; we also report our results with the bounding boxes predicted by Pix2Pose~\cite{park-iccv19-pix2pose}.}
    \label{tab:tless}
\end{table}
